HyperNeRF: A Higher-Dimensional Representation for Topologically Varying Neural Radiance Fields

Neural Radiance Fields (NeRF) are able to reconstruct scenes with unprecedented fidelity, and various recent works have extended NeRF to handle dynamic scenes. A common approach to reconstruct such non-rigid scenes is through the use of a learned deformation field mapping from coordinates in each input image into a canonical template coordinate space. However, these deformation-based approaches struggle to model changes in topology, as topological changes require a discontinuity in the deformation field, but these deformation fields are necessarily continuous. We address this limitation by lifting NeRFs into a higher dimensional space, and by representing the 5D radiance field corresponding to each individual input image as a slice through this "hyper-space". Our method is inspired by level set methods, which model the evolution of surfaces as slices through a higher dimensional surface. We evaluate our method on two tasks: (i) interpolating smoothly between "moments", i.e., configurations of the scene, seen in the input images while maintaining visual plausibility, and (ii) novel-view synthesis at fixed moments. We show that our method, which we dub HyperNeRF, outperforms existing methods on both tasks. Compared to Nerfies, HyperNeRF reduces average error rates by 4.1% for interpolation and 8.6% for novel-view synthesis, as measured by LPIPS. Additional videos, results, and visualizations are available at https://hypernerf.github.io.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> figures/interp_results_combined.tex <==
\definecolor{bestcolor}{rgb}{0.85, 0.113, 0.188}

\renewcommand{\animage}[2]{\includegraphics[width=1.65cm,clip,trim=#1]{images/interp_images_v3/#2}}

\begin{figure*}[t!]
    \setlength{\tabcolsep}{0.5pt}
    \renewcommand{\arraystretch}{0.25}
    \begin{tabular}{ccccccccccc}
    
        % \multirow{2}{*}[0.2in]{\makebox[20pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Chicken}}}} \hspace{-7pt}} &
        % \animage{45 130 45 90}{chickchicken.left.jpg} &
        % \animage{45 130 45 90}{chickchicken.right.jpg} &
        % \animage{45 130 45 90}{chickchicken.nerf.target.jpg} &
        % \animage{45 130 45 90}{chickchicken.hypernerf-bs-2d.pred.jpg} &
        % \animage{45 130 45 90}{chickchicken.hypernerf-ap-2d.pred.jpg} &
        % \animage{45 130 45 90}{chickchicken.no-deform.pred.jpg} &
        % \animage{45 130 45 90}{chickchicken.nerfies-elastic.pred.jpg} &
        % \animage{45 130 45 90}{chickchicken.neuralvolumes.pred.jpg} &
        % \animage{45 130 45 94}{chickchicken.nsff.pred.jpg} &
        % \animage{45 130 45 90}{chickchicken.nerf.pred.jpg} \\
        % & & & &
        % \animage{45 130 45 90}{chickchicken.hypernerf-bs-2d.error.jpg} &
        % \animage{45 130 45 90}{chickchicken.hypernerf-ap-2d.error.jpg} &
        % \animage{45 130 45 90}{chickchicken.no-deform.error.jpg} &
        % \animage{45 130 45 90}{chickchicken.nerfies-elastic.error.jpg} &
        % \animage{45 130 45 90}{chickchicken.neuralvolumes.error.jpg} &
        % \animage{45 130 45 94}{chickchicken.nsff.error.jpg} &
        % \animage{45 130 45 90}{chickchicken.nerf.error.jpg} \\
        
        \multirow{2}{*}[0.1in]{\makebox[20pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Fist}}}} \hspace{-7pt}} &
        \animage{20 170 80 140}{hand1-dense-v2.left.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.right.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.nerf.target.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.hypernerf-bs-2d.pred.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.hypernerf-ap-2d.pred.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.no-deform.pred.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.nerfies-elastic.pred.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.neuralvolumes.pred.jpg} &
        \animage{20 170 80 144}{hand1-dense-v2.nsff.pred.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.nerf.pred.jpg} \\
        & & & &
        \animage{20 170 80 140}{hand1-dense-v2.hypernerf-bs-2d.error.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.hypernerf-ap-2d.error.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.no-deform.error.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.nerfies-elastic.error.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.neuralvolumes.error.jpg} &
        \animage{20 170 80 144}{hand1-dense-v2.nsff.error.jpg} &
        \animage{20 170 80 140}{hand1-dense-v2.nerf.error.jpg} \\
        
        
        \multirow{2}{*}[0.35in]{\makebox[20pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Slice Banana}}}} \hspace{-7pt}} &
        \animage{35 150 25 100}{slice-banana.left.jpg} &
        \animage{35 150 25 100}{slice-banana.right.jpg} &
        \animage{35 150 25 100}{slice-banana.nerf.target.jpg} &
        \animage{35 150 25 100}{slice-banana.hypernerf-bs-2d.pred.jpg} &
        \animage{35 150 25 100}{slice-banana.hypernerf-ap-2d.pred.jpg} &
        \animage{35 150 25 100}{slice-banana.no-deform.pred.jpg} &
        \animage{35 150 25 100}{slice-banana.nerfies-elastic.pred.jpg} &
        \animage{35 150 25 100}{slice-banana.neuralvolumes.pred.jpg} &
        \animage{35 150 25 100}{slice-banana.nsff.pred.jpg} &
        \animage{35 150 25 100}{slice-banana.nerf.pred.jpg} \\
        & & & &
        \animage{35 150 25 100}{slice-banana.hypernerf-bs-2d.error.jpg} &
        \animage{35 150 25 100}{slice-banana.hypernerf-ap-2d.error.jpg} &
        \animage{35 150 25 100}{slice-banana.no-deform.error.jpg} &
        \animage{35 150 25 100}{slice-banana.nerfies-elastic.error.jpg} &
        \animage{35 150 25 100}{slice-banana.neuralvolumes.error.jpg} &
        \animage{35 150 25 100}{slice-banana.nsff.error.jpg} &
        \animage{35 150 25 100}{slice-banana.nerf.error.jpg} \\
        
        % \multirow{2}{*}[0.13in]{\makebox[20pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Torch}}}} \hspace{-7pt}} &
        % \animage{80 90 0 140}{torchocolate.left.jpg} &
        % \animage{80 90 0 140}{torchocolate.right.jpg} &
        % \animage{80 90 0 140}{torchocolate.nerf.target.jpg} &
        % \animage{80 90 0 140}{torchocolate.hypernerf-bs-2d.pred.jpg} &
        % \animage{80 90 0 140}{torchocolate.hypernerf-ap-2d.pred.jpg} &
        % \animage{80 90 0 140}{torchocolate.no-deform.pred.jpg} &
        % \animage{80 90 0 140}{torchocolate.nerfies-elastic.pred.jpg} &
        % \animage{80 90 0 140}{torchocolate.neuralvolumes.pred.jpg} &
        % \animage{80 90 0 140}{torchocolate.nsff.pred.jpg} &
        % \animage{80 90 0 140}{torchocolate.nerf.pred.jpg} \\
        % & & & &
        % \animage{80 90 0 140}{torchocolate.hypernerf-bs-2d.error.jpg} &
        % \animage{80 90 0 140}{torchocolate.hypernerf-ap-2d.error.jpg} &
        % \animage{80 90 0 140}{torchocolate.no-deform.error.jpg} &
        % \animage{80 90 0 140}{torchocolate.nerfies-elastic.error.jpg} &
        % \animage{80 90 0 140}{torchocolate.neuralvolumes.error.jpg} &
        % \animage{80 90 0 140}{torchocolate.nsff.error.jpg} &
        % \animage{80 90 0 140}{torchocolate.nerf.error.jpg} \\
        
         \multirow{2}{*}[0.13in]{\makebox[20pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Lemon}}}} \hspace{-7pt}} &
        \animage{120 40 90 20}{cut-lemon1.left.jpg} &
        \animage{80 40 130 20}{cut-lemon1.right.jpg} &
        \animage{80 40 130 20}{cut-lemon1.nerf.target.jpg} &
        \animage{80 40 130 20}{cut-lemon1.hypernerf-bs-2d.pred.jpg} &
        \animage{80 40 130 20}{cut-lemon1.hypernerf-ap-2d.pred.jpg} &
        \animage{80 40 130 20}{cut-lemon1.no-deform.pred.jpg} &
        \animage{80 40 130 20}{cut-lemon1.nerfies-elastic.pred.jpg} &
        \animage{80 40 130 20}{cut-lemon1.neuralvolumes.pred.jpg} &
        \animage{80 36 130 20}{cut-lemon1.nsff.pred.jpg} &
        \animage{80 40 130 20}{cut-lemon1.nerf.pred.jpg} \\
        & & & &
        \animage{80 40 130 20}{cut-lemon1.hypernerf-bs-2d.error.jpg} &
        \animage{80 40 130 20}{cut-lemon1.hypernerf-ap-2d.error.jpg} &
        \animage{80 40 130 20}{cut-lemon1.no-deform.error.jpg} &
        \animage{80 40 130 20}{cut-lemon1.nerfies-elastic.error.jpg} &
        \animage{80 40 130 20}{cut-lemon1.neuralvolumes.error.jpg} &
        \animage{80 36 130 20}{cut-lemon1.nsff.error.jpg} &
        \animage{80 40 130 20}{cut-lemon1.nerf.error.jpg} \\
        
            
        % \multirow{2}{*}[0.35in]{\makebox[20pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Expressions 1}}}} \hspace{-7pt}} &
        % % \makebox[20pt]{\raisebox{42pt}{\rotatebox[origin=c]{90}{\textsc{Expressions 1}}}} \hspace{-7pt} &
        % \animage{30 120 30 60}{ricardo-expressions.left.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.right.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.nerf.target.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.hypernerf-bs-2d.pred.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.hypernerf-ap-2d.pred.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.no-deform.pred.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.nerfies-elastic.pred.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.neuralvolumes.pred.jpg} &
        % \animage{30 120 30 58}{ricardo-expressions.nsff.pred.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.nerf.pred.jpg} \\
        % & & & &
        % \animage{30 120 30 60}{ricardo-expressions.hypernerf-bs-2d.error.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.hypernerf-ap-2d.error.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.no-deform.error.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.nerfies-elastic.error.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.neuralvolumes.error.jpg} &
        % \animage{30 120 30 58}{ricardo-expressions.nsff.error.jpg} &
        % \animage{30 120 30 60}{ricardo-expressions.nerf.error.jpg} \\
        
        % \multirow{2}{*}[0.35in]{\makebox[20pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Expressions 2}}}} \hspace{-7pt}} &
        % \animage{75 140 40 100}{keunhong-expressions.left.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.right.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.nerf.target.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.hypernerf-bs-2d.pred.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.hypernerf-ap-2d.pred.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.no-deform.pred.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.nerfies-elastic.pred.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.neuralvolumes.pred.jpg} &
        % \animage{67 128 36 92}{keunhong-expressions.nsff.pred.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.nerf.pred.jpg} \\
        % & & & &
        % \animage{75 140 40 100}{keunhong-expressions.hypernerf-bs-2d.error.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.hypernerf-ap-2d.error.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.no-deform.error.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.nerfies-elastic.error.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.neuralvolumes.error.jpg} &
        % \animage{67 128 36 92}{keunhong-expressions.nsff.error.jpg} &
        % \animage{75 140 40 100}{keunhong-expressions.nerf.error.jpg} \\
        
        
        \multirow{2}{*}[0.35in]{\makebox[20pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Expressions 3}}}} \hspace{-7pt}} &
        \animage{25 80 30 81}{aleks-expressions.left.jpg} &
        \animage{25 80 30 81}{aleks-expressions.right.jpg} &
        \animage{25 80 30 81}{aleks-expressions.nerf.target.jpg} &
        \animage{25 80 30 81}{aleks-expressions.hypernerf-bs-2d.pred.jpg} &
        \animage{25 80 30 81}{aleks-expressions.hypernerf-ap-2d.pred.jpg} &
        \animage{25 80 30 81}{aleks-expressions.no-deform.pred.jpg} &
        \animage{25 80 30 81}{aleks-expressions.nerfies-elastic.pred.jpg} &
        \animage{25 80 30 81}{aleks-expressions.neuralvolumes.pred.jpg} &
        \animage{25 80 30 81}{aleks-expressions.nsff.pred.jpg} &
        \animage{25 80 30 81}{aleks-expressions.nerf.pred.jpg} \\
        & & & &
        \animage{25 80 30 81}{aleks-expressions.hypernerf-bs-2d.error.jpg} &
        \animage{25 80 30 81}{aleks-expressions.hypernerf-ap-2d.error.jpg} &
        \animage{25 80 30 81}{aleks-expressions.no-deform.error.jpg} &
        \animage{25 80 30 81}{aleks-expressions.nerfies-elastic.error.jpg} &
        \animage{25 80 30 81}{aleks-expressions.neuralvolumes.error.jpg} &
        \animage{25 80 30 81}{aleks-expressions.nsff.error.jpg} &
        \animage{25 80 30 81}{aleks-expressions.nerf.error.jpg} \\
        
        \multirow{2}{*}[0.2in]{\makebox[10pt]{\raisebox{25pt}{\rotatebox[origin=c]{90}{\textsc{Teapots}}}} \hspace{-7pt}} &
        \animage{40 65 80 200}{aleks-teapot.left.jpg} &
        \animage{40 65 80 200}{aleks-teapot.right.jpg} &
        \animage{40 65 80 200}{aleks-teapot.nerf.target.jpg} &
        \animage{40 65 80 200}{aleks-teapot.hypernerf-bs-2d.pred.jpg} &
        \animage{40 65 80 200}{aleks-teapot.hypernerf-ap-2d.pred.jpg} &
        \animage{40 65 80 200}{aleks-teapot.no-deform.pred.jpg} &
        \animage{40 65 80 200}{aleks-teapot.nerfies-elastic.pred.jpg} &
        \animage{40 65 80 200}{aleks-teapot.neuralvolumes.pred.jpg} &
        \animage{40 65 80 200}{aleks-teapot.nsff.pred.jpg} &
        \animage{40 65 80 200}{aleks-teapot.nerf.pred.jpg} \\
        & & & &
        \animage{40 65 80 200}{aleks-teapot.hypernerf-bs-2d.error.jpg} &
        \animage{40 65 80 200}{aleks-teapot.hypernerf-ap-2d.error.jpg} &
        \animage{40 65 80 200}{aleks-teapot.no-deform.error.jpg} &
        \animage{40 65 80 200}{aleks-teapot.nerfies-elastic.error.jpg} &
        \animage{40 65 80 200}{aleks-teapot.neuralvolumes.error.jpg} &
        \animage{40 65 80 200}{aleks-teapot.nsff.error.jpg} &
        \animage{40 65 80 200}{aleks-teapot.nerf.error.jpg} \\
        
        \\[2pt]
        
        & 
        {\smaller Reference 1} & 
        {\smaller Reference 2} & 
        {\smaller \makecell{Interpolated\\(GT)}} & 
        {\smaller \makecell{HyperNeRF\\(DS)}} &
        {\smaller \makecell{HyperNeRF\\(AP)}} &
        {\smaller No Deform} &
        {\smaller Nerfies} &
        {\smaller \makecell{Neural\\Volumes}} &
        {\smaller NSFF} &
        {\smaller NeRF}
        \\
    \end{tabular}
    \vspace{-6pt}
    \caption{Qualitative comparisons of our method, ablations, and baselines on the interpolation dataset (See \secref{sec:evaluation_quantitative}). The interpolated frame is rendered by linearly interpolating between the latent codes of the two reference frames. The bottom row of each sequence shows the absolute error. Baselines shown are: Nerfies~\cite{park2020nerfies}, Neural Volumes~\cite{lombardi2019neural}, NSFF~\cite{li2020nsff}, and NeRF~\cite{mildenhall2020nerf}. See \secref{sec:evaluation_interpolation} for details.}
    \label{fig:interp_results_combined}
    \vspace{-12pt}
\end{figure*}

